Instance Based Approximations to Profile Maximum Likelihood

In this paper we provide a new efficient algorithm for approximately computing the profile maximum likelihood (PML) distribution, a prominent quantity in symmetric property estimation. We provide an algorithm which matches the previous best known efficient algorithms for computing approximate PML distributions and improves when the number of distinct observed frequencies in the given instance is small. We achieve this result by exploiting new sparsity structure in approximate PML distributions and providing a new matrix rounding algorithm, of independent interest. Leveraging this result, we obtain the first provable computationally efficient implementation of PseudoPML, a general framework for estimating a broad class of symmetric properties. Additionally, we obtain efficient PML-based estimators for distributions with small profile entropy, a natural instance-based complexity measure. Further, we provide a simpler and more practical PseudoPML implementation that matches the best-known theoretical guarantees of such an estimator and evaluate this method empirically.

==> anari.tex <==
\makeatletter


% -- Options

\RequirePackage{options}

\options{
	/opts/.new family,
	/opts/colors/.new toggle=true,
	/opts/fonts/.new toggle=true,
	/opts/math/.new toggle=true,
	/opts/theorems/.new toggle=true,
	/opts/macros/.new toggle=true,
	/opts/graphics/.new toggle=true,
	/opts/tools/.new toggle=true,
	/opts/typesetting/.new toggle=true,
	/opts/biblio/.new toggle=true
}
\options{/opts}

\providetoggle{presentation}
\@ifclassloaded{beamer}{\toggletrue{presentation}}{\togglefalse{presentation}}

% -- Packages

\iftoggle{/opts/math}{
	\RequirePackage{amsmath}
	\RequirePackage{amssymb}
	\RequirePackage{bm}
	\RequirePackage{dsfont}
	\RequirePackage{mathtools}
}{}

\iftoggle{/opts/theorems}{
	\RequirePackage{amsthm}
}{}

\iftoggle{/opts/graphics}{
	\RequirePackage{tikz}
	\RequirePackage{tikz-3dplot}
	\RequirePackage{tcolorbox}
	\RequirePackage{pgfplots}
	\RequirePackage{tcolorbox}
	\pgfplotsset{compat=newest}
}{}

\iftoggle{/opts/tools}{
	\RequirePackage[ruled]{algorithm2e}
	\RequirePackage{datatool}
	\RequirePackage[super]{nth}
	\RequirePackage{scalerel}
	\iftoggle{presentation}{}{
		\RequirePackage[shortlabels]{enumitem}
	}
}{}

\iftoggle{/opts/fonts}{
	\iftoggle{presentation}{}{
		\RequirePackage[sc]{mathpazo}
	}
}{}

\iftoggle{/opts/biblio}{
	\iftoggle{presentation}{}{
		\RequirePackage[backend=biber, style=alphabetic, maxbibnames=99, maxcitenames=99, url=false]{biblatex}
	}
}

\iftoggle{/opts/colors}{
	\newcommand{\declarecolor}[2]{\@ifundefined{\string\color@#1}{\definecolor{#1}{RGB}{#2}\expandafter\newcommand\csname #1\endcsname[1]{\textcolor{#1}{##1}}}{}}
	\declarecolor{Black}{0, 0, 0}
	\declarecolor{White}{255, 255, 255}
	\declarecolor{Gray}{127, 127, 127}
	\declarecolor{LightGray}{216, 216, 216}
	\declarecolor{Orange}{237, 125, 49}
	\declarecolor{LightOrange}{251,229, 214}
	\declarecolor{Yellow}{255, 192, 0}
	\declarecolor{LightYellow}{255, 242, 200}
	\declarecolor{Blue}{91, 155, 213}
	\declarecolor{LightBlue}{222, 235, 247}
	\declarecolor{Green}{112, 173, 71}
	\declarecolor{LightGreen}{226, 240, 217}
	\declarecolor{Navy}{68, 114, 196}
	\declarecolor{LightNavy}{218, 227, 243}
	
	\newcommand{\declareperson}[1]{%
		\expandafter\newcommand\csname#1\endcsname[1]{\textcolor{Orange}{#1: ##1}}%
	}
}{}

\iftoggle{/opts/graphics}{
	\RequirePackage{tikzsymbols}
	
	\usetikzlibrary{decorations}
	\usetikzlibrary{decorations.pathreplacing}
	\usetikzlibrary{decorations.markings}
	\usetikzlibrary{fit}
	\usetikzlibrary{intersections}
	\usetikzlibrary{matrix}
	\usetikzlibrary{overlay-beamer-styles}
	\usetikzlibrary{patterns}
	\usetikzlibrary{shapes}
	\usetikzlibrary{tikzmark}
	\usetikzlibrary{hobby}
	
	\usepgflibrary{arrows.meta}
	
	\tcbuselibrary{skins}
	\tcbuselibrary{raster}
	
	\usepgfplotslibrary{patchplots}
		
	\pgfdeclarelayer{background}
	\pgfdeclarelayer{foreground}
	\pgfsetlayers{background,main,foreground}
	\tikzstyle{na}=[baseline=-0.5ex]
	\tikzset{onslide/.code args={<#1>#2}{%
	  \only<#1>{\pgfkeysalso{#2}}
	}}
	\tikzset{temporal/.code args={<#1>#2#3#4}{%
	  \temporal<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}{\pgfkeysalso{#4}}
	}}
		
	\pgfplotsset{colormap={WhiteOrange}{
		color=(White)
		color=(Orange)
	}}
	\pgfplotsset{colormap={NavyOrange}{
		color=(LightNavy)
		color=(Orange)
	}}
	\pgfplotsset{colormap={WhiteNavy}{
		color=(White)
		color=(Navy)
	}}
	\pgfplotsset{colormap={WhiteBlack}{
		color=(White)
		color=(Black)
	}}
		
	\newcommand*{\Pic}[2][]{\begin{tikzpicture}\pic[#1]{#2};\end{tikzpicture}}
	\newcommand*{\sPic}[2]{\scalebox{#1}{\Pic{#2}}}
	\newcommand*{\cPic}[2][]{\begin{center}\Pic[#1]{#2}\end{center}}
	
	\newcommand{\rounded}[2][0.7ex]{%
		\begin{tikzpicture}
			\node[inner sep=0ex, draw=White, line width=0ex, opacity=0.] (a) {#2};
			\clip[rounded corners=#1] (a.south west) rectangle (a.north east);
			\node[inner sep=0ex] (a) {#2};
		\end{tikzpicture}%
	}
	
	\newcommand*{\tnode}[2]{\tikzmarknode{#1}{#2}}
}{}

\iftoggle{/opts/typesetting}{
	\iftoggle{presentation}{
	}{
		\RequirePackage{microtype}
		\RequirePackage[noblocks]{authblk}
		\RequirePackage{parskip}
		\RequirePackage{fullpage}
	}
	\RequirePackage{hyperref}
	\RequirePackage[capitalize, nameinlink]{cleveref}
	
	\iftoggle{/opts/colors}{
		\hypersetup{
			colorlinks=true,
			pdfpagemode=UseNone,
			citecolor=Green,
			linkcolor=Navy,
			urlcolor=Black
		}
	}{}
}{}

\iftoggle{/opts/theorems}{
	\iftoggle{presentation}{}{
		\theoremstyle{plain}
		\newtheorem{theorem}{Theorem}
		\newtheorem{lemma}[theorem]{Lemma}
		\newtheorem{corollary}[theorem]{Corollary}
		\newtheorem{proposition}[theorem]{Proposition}
		\newtheorem{fact}[theorem]{Fact}
		\newtheorem{conjecture}[theorem]{Conjecture}
		\newtheorem*{conjecture*}{Conjecture}
		
		\theoremstyle{definition}
		\newtheorem{definition}[theorem]{Definition}
		
		\theoremstyle{remark}
		\newtheorem{remark}[theorem]{Remark}
		\newtheorem{example}[theorem]{Example}
	}
}{}

\iftoggle{/opts/macros}{
	\providecommand{\given}{}
	\newcommand\GivenSymbol[1][]{%
		\nonscript\:#1\vert%
		\allowbreak%
		\nonscript\:%
		\mathopen{}%
	}
	\newcommand{\declaredelims}[3]{%
		\expandafter\DeclarePairedDelimiterX\csname#1\endcsname[1]{#2}{#3}{\renewcommand\given{\GivenSymbol[\delimsize]}##1}%
	}
	
	\declaredelims{set}\{\}
	\declaredelims{card}\lvert\rvert
	\declaredelims{abs}\lvert\rvert
	\declaredelims{norm}\lVert\rVert
	\declaredelims{dotp}\langle\rangle
	\declaredelims{tuple}\lparen\rparen
	\declaredelims{parens}\lparen\rparen
	\declaredelims{bracks}\lbrack\rbrack
	
	\newcommand{\declarenameddelims}[4]{%
		\expandafter\DeclarePairedDelimiterXPP\csname#1\endcsname[1]{#2}{#3}{#4}{}{\renewcommand\given{\GivenSymbol[\delimsize]}##1}%
		\expandafter\DeclarePairedDelimiterXPP\csname#1X\endcsname[2]{#2_{##1}}{#3}{#4}{}{\renewcommand\given{\GivenSymbol[\delimsize]}##2}%
	}
	
	
	\let\Pr\relax
	\declarenameddelims{Pr}{\mathbb{P}}\lbrack\rbrack
	\declarenameddelims{Ex}{\mathbb{E}}\lbrack\rbrack
	
	\newcommand*{\eval}[1]{\left.#1\right\rvert}
	
	\iftoggle{presentation}{%
		\newcommand*{\mathdouble}[1]{\mathds{#1}}%
	}{%
		\newcommand*{\mathdouble}[1]{\mathbb{#1}}%
	}
	
	\let\Q\relax
	\newcommand*{\Q}{{\mathdouble{Q}}}
	\let\N\relax
	\newcommand*{\N}{{\mathdouble{N}}}
	\let\Z\relax
	\newcommand*{\Z}{{\mathdouble{Z}}}
	\let\R\relax
	\newcommand*{\R}{{\mathdouble{R}}}
	\let\C\relax
	\newcommand*{\C}{{\mathdouble{C}}}
	\let\1\relax
	\newcommand*{\1}{{\mathds{1}}}
	\let\l\relax
	\newcommand*{\l}{{\ell}}
	
	\let\poly\relax
	\DeclareMathOperator{\poly}{poly}
	\DeclareMathOperator{\supp}{supp}
	\DeclareMathOperator{\conv}{conv}
	\DeclareMathOperator{\rank}{rank}
	\let\Im\relax
	\DeclareMathOperator{\Im}{Im}
	\let\Re\relax
	\DeclareMathOperator{\Re}{Re}
}{}
\makeatother


==> final_rounding.tex <==
\renewcommand{\bttpo}{(\btt+1)}
\renewcommand{\bSp}{\textbf{B}}
\renewcommand{\bS}{\textbf{C}}
\renewcommand{\boo}{t}
\subsection{Combining everything together}\label{subsec:combine}
Here we provide an efficient algorithm to compute an $\expo{-O(k \log n)}$ approximate PML distribution. 
\kiran{Rewrite a short form of this result}
The main contribution of this section is to define a probability discretization set $\bR$ that guarantees existence of a discrete pseudo-distrbution $\bq$ with respect to $\bR$ that is also an $\expo{\sqrt{n}\log n}$ approximate PML pseudo-distribution. We further use this probability discretization set $\bR$ and combine it with results from the previous two sections to finally output an $\expo{\sqrt{n}\log n}$ approximate PML distribution. In this direction, we first provide definition of $\bR$ that has desired guarantees and such a set $\bR$ was already constructed in \cite{CSS19} and we formally state results from \cite{CSS19} that help us define such a set $\bR$. 



\begin{lemma}[Lemma 4.1 in \cite{CSS19}]\label{lemminmain}
	For any profile $\phi \in \Phi^{n}$, there exists a distribution $\bp'' \in \simplex$ such that $\bp''$ is an $\expo{-6}$-approximate PML distribution and $\min_{x \in \bX:\bp''_x \neq 0}\bp''_x \geq \frac{1}{2n^2}$.
\end{lemma} 
The above result allows to define a probability discretization set ($\bR$) and we define $\bR\defeq\{(1+\epso)^{1-i}\}_{i \in [\boo]}$ for some $\epso \in (0,1)$, where $\boo=O(\frac{\log n}{\epso})$ is the smallest integer such that $\frac{1}{4n^2} \leq (1+\epso)^{1-\boo}\leq \frac{1}{2n^2}$. We next state a result in \cite{CSS19} that captures the effect of this discretization.
\renewcommand{\bp}{\textbf{p}}
\begin{lemma}[Lemma 4.4 in \cite{CSS19}]\label{lem:probdisc}
	For any profile $\phi \in \Phi^{n}$ and distribution $\bp \in \simplex$, its discrete pseudo-distribution $\bq=\disc(\bp) \in \dsimplex$ satisfies:
	$$\probpml(\bp,\phi) \geq \probpml(\bq,\phi) \geq \expo{-\epso n}\probpml(\bp,\phi)~.$$
\end{lemma}

\renewcommand{\boo}{\ell}
%\renewcommand{\epso}{\epsilon}

We are now ready to state our final algorithm. Following this algorithm, we prove that it returns an approximate PML distribution.

%\kiran{Uncomment algorithm here.}
\begin{algorithm}[H]
	\caption{Algorithm for approximate PML}\label{euclid}
	\begin{algorithmic}[1]
		\Procedure{Approximate PML}{$\phi,\bR$}
		\State {\bf Input}: Profile $\phi \in \Phi^n$ and probability discretization set $\bR$.
		\State {\bf Output}: A distribution $\bpapprox$.
		\State Solve $\bSp=\argmax_{\bS\in \bZfrac} \log \bg(\bS)$. 
		\State Use \Cref{alg:rounding} to round the fractional solution $\bSp$ to integral solution $\bSext \in \bZext$.
		\State Construct discrete pseudo-distribution $\qext$ with respect to $\bSext$ (See \Cref{defn:distS}).
		%by assigning $(\bS \onevec)_{i}$ number of domain elements probability $\ri$ 
		\State \textbf{return} $\bpapprox\defeq \frac{\qext}{\|\qext\|_1}$.
		\EndProcedure
	\end{algorithmic}
	\label{alg:final}
\end{algorithm}
\renewcommand{\pml}{\textbf{p}_{\mathrm{pml}}}
%\apmlthm*
\begin{proof}
	Choose $\epso=\frac{k}{n}$ and let the probability discretization space $\bR\defeq\{(1+\frac{1}{\sqrt{n}})^{1-i}\}_{i \in [\boo]}$ and $\boo\defeq |\bR|$ be the smallest integer such that $\frac{1}{2n^2} \geq (1+\frac{1}{\sqrt{n}})^{1-\boo} \geq \frac{1}{4n^2}$ and therefore $\boo \in O(\frac{n \log n}{k})$. The minimum non-zero probability of the set $\bR$ is $\rmin \geq \frac{1}{4n^2}$.
	
	Given profile $\phi$, let $\pml$ be the PML distribution. Define $\dpml \defeq \floor{\pml}_{\bR}$ and by \Cref{lem:probdisc} (and choice of $\epso$) we have,
	\begin{equation}\label{eq:ddone}
	\probpml(\dpml,\phi)\geq \expo{- O(k \log n)}\probpml(\pml,\phi)~.
	\end{equation}
	
	\begin{comment}
	Define $\bSp'\defeq \max_{\bS \in \zdpml}\bg(\bS)$, then by \Cref{pmlprob:approx} we have,
	\begin{equation}\label{eq:ddtwo}
	\probpml(\dpml,\phi) \leq \expo{\bigO{k \log \frac{\Ns}{k}}} \cdot \cphi \cdot \bg(\bSp')
	\end{equation}
	\end{comment}
	
	Let $\bSp \defeq \argmax_{\bS\in \bZfrac}\bg(\bS)$, then by \Cref{lem:dpmlapprox} we have,
	\begin{equation}\label{eq:ddtwo}
	\max_{\bq \in \dsimplex}\probpml(\bp,\phi) \leq \expo{\bigO{k \log \frac{\Ns}{k}}} \cdot \cphi \cdot \bg(\bSp)~.
	\end{equation}
	Note $\dpml \in \dsimplex$, therefore $\probpml(\dpml,\phi) \leq \max_{\bq \in \dsimplex}\probpml(\bq,\phi)$ and further combined with equations \ref{eq:ddone} and \ref{eq:ddtwo} we have,
	\begin{equation}\label{eq:ddthree}
	\probpml(\pml,\phi) \leq \expo{\bigO{k \log \frac{\Ns}{k} +k \log n}} \cdot \cphi \cdot \bg(\bSp)~.
	\end{equation}
	Let $\bSext$ and $\bRext$ be the solution returned by \Cref{alg:rounding}, then by the second condition of \Cref{thm:stepthree} we have,
	\begin{equation}\label{eq:ddfour}
	\bg(\bSext) \geq \expo{-O(k\log \frac{1}{\rmin})} \bg(\bSp)
	\end{equation}
	Combining equations \ref{eq:ddthree} and \ref{eq:ddfour} we have,
	\begin{equation}\label{eq:z}
	\probpml(\pml,\phi) \leq \expo{\bigO{k \log \frac{\Ns}{k} +k \log n + k\log \frac{1}{\rmin} }} \cdot \cphi \cdot \bg(\bSext)~.
	\end{equation}
	 By \Cref{lemminmain}, up to constant multiplicative loss we can assume that the minimum non-zero probability value of our approximate PML distribution is at least $\frac{1}{4n^2}$ and therefore the support $\Ns \leq 4n^2$. Further combined with $\rmin \geq \frac{1}{4n^2}$, the above equation simplifies to,
	\begin{equation}\label{eq:ddfive}
	\probpml(\pml,\phi) \leq \expo{\bigO{k \log n }} \cdot \cphi \cdot \bg(\bSext)~.
	\end{equation}
	By the first condition of \Cref{thm:stepthree} we have $\bSext \in \bZext$. Let $\qext$ be the discrete pseudo-distribution with respect to $\bSext$, then the condition $\bSext \in \bZext$ further implies $\bSext \in \bZqext$ and combined with \Cref{pmlprob:approx} we have,
	\begin{equation}\label{eq:ddsix}
	\expo{-O(k \log (\Ns+n))}\cdot	\cphi \cdot	\bg(\bSext) \leq \probpml(\qext,\phi)
	\end{equation}
	Combining equations \ref{eq:ddfive}, \ref{eq:ddsix} and $\Ns \leq 4n^2$ we have,
	\begin{equation}\label{eq:ddseven}
	\probpml(\qext,\phi) \geq \expo{-\bigO{k \log n }} \probpml(\pml,\phi)~.
	\end{equation}
	Define $\bpapprox\defeq \frac{\qext}{\|\qext\|_1}$, then $\bpapprox$ is a distribution, $\probpml(\bpapprox,\phi) \geq \probpml(\qext,\phi)$ (because $\qext$ is a pseudo-distribution and $\|\qext\|_1\leq 1$) and combined with \Cref{eq:ddseven} we get,
	\begin{equation}
	\probpml(\bpapprox,\phi) \geq \expo{-\bigO{k \log n }} \probpml(\pml,\phi)~.
	\end{equation}
	Therefore $\bpapprox$ is an $\expo{-\bigO{k \log n }}$-approximate PML distribution. 
	Note all the steps in our algorithm can be implemented in polynomial time and therefore we conclude the proof.
\end{proof}

==> missingproofs.tex <==
\subsection{Missing Proofs from \Cref{subsec:algmain}}\label{subsec:missing}
Here we provide the proofs for all the lemmas and theorems in \Cref{subsec:algmain}
\begin{proof}[Proof of \Cref{lem:structured}]
	Without loss of generality assume $w_{0} \geq w_{1} \geq w_{2} \dots \geq w_{k}$. Let $a\defeq \sum_{j\in \ztbtt}x_{j} $, we invoke \Cref{alg:structurerounding} with inputs $(x,w,a)$. Let $s\in \Z^{a}$ and $z\in \R^{\ztbtt \times \ztbtt}$ be the output of \Cref{alg:structurerounding}. We now provide the proof for the three conditions in the lemma.
	
	{\bf Condition 1}: By construction of \Cref{alg:structurerounding}, for any $s \in \{s_{i}\}_{i\in [1,a]}$ we have $\sum_{j\in \ztbtt}z_{s,j}=1$ (Line 6) and for any other $s \in \ztbtt \backslash \{s_{i}\}_{i\in [1,a]}$ we have $\sum_{j\in \ztbtt}z_{s,j}=0$. Therefore the first part of condition 1 holds.
	
	For any $j \in \ztbtt$, one of the following two cases holds,
	\begin{enumerate}
		\item If $j\in \{s_{i}\}_{i\in [1,a]}$ and in this case let $i \in [1,a]$ be such that $s_{i}=j$. By line 6 (third case) of the algorithm we have,
		\begin{equation}\label{eq:fone}
		z_{s_{i-1},j}=1-\left(\sum_{j'\leq s_{i-1}}x_{j'}-(i-2)+\sum_{s_{i-1}<j'<s_{i}}x_{j'} \right)=(i-1)-\sum_{j'<s_{i}}x_{j'}~.
		\end{equation}
		We now analyze the term $\sum_{i'\in \ztbtt}z_{i',j}$,
		$$\sum_{i'\in \ztbtt}z_{i',j}=z_{s_{i},j}+z_{s_{i-1},j}=\sum_{j'\leq s_{i}}x_{j'}-(i-1)+(i-1)-\sum_{j'<s_{i}}x_{j'}=x_{s_{i}}=x_{j}~.$$
		The first equality follows because for $i' \in \ztbtt \backslash \{s_{i},s_{i-1}\}$ we have $z_{i',j}=0$ and this follows by the second and third case in line 6 of the algorithm. In the second equality we substituted values for $z_{s_{i},s_{i}}$ and $z_{s_{i-1},s_{i}}$ using second case (Line 6) and \Cref{eq:fone} respectively.
		\item Else $j\in \ztbtt\backslash \{s_{i}\}_{i\in [1,a]}$, and in this case let $i \in [1,a]$ be such that $s_{i}<j<s_{i+1}$. Then by the first case in line 6 of the algorithm we have,
		$$\sum_{i'\in \ztbtt}z_{i',j}=z_{s_{i},j}=x_{j}~.$$
	\end{enumerate}
	{\bf Condition 2:} Consider $\sum_{i\in \ztbtt}\left(\sum_{j\in \ztbtt}z_{i,j}\right)w_{i}$,
	\begin{equation}\label{eq:gone}
	\begin{split}
	\sum_{i\in \ztbtt}\left(\sum_{j\in \ztbtt}z_{i,j}\right)w_{i}&=\sum_{i\in [1,a]}\left(\sum_{s_{i}\leq j  \leq s_{i+1}}z_{\si,j}\right)w_{\si} \leq \sum_{i\in [1,a]}\sum_{s_{i}\leq j  \leq s_{i+1}}z_{\si,j}(w_{j}+w_{s_{i}}-w_{s_{i+1}})\\
	&\leq \sum_{i\in [1,a]}\sum_{s_{i}\leq j  \leq s_{i+1}}z_{\si,j}w_{j}+\sum_{i\in [1,a]}\sum_{s_{i}\leq j  \leq s_{i+1}}z_{\si,j}(w_{s_{i}}-w_{s_{i+1}})\\
	&= \sum_{i\in [1,a]}\sum_{j  \in \ztbtt}z_{\si,j}w_{j}+\sum_{i\in [1,a]}\sum_{s_{i}\leq j  \leq s_{i+1}}z_{\si,j}(w_{s_{i}}-w_{s_{i+1}})~.\\
	\end{split}
	\end{equation}
	The first equality follows because rest of the other entries are zero. In the second inequality we used $j \leq s_{i+1}$ and therefore $w_{j} \geq w_{s_{i+1}}$ by our assumption at the beginning of the proof. In the remainder, we simplify both the terms. Consider the first term in the final expression above,
	\begin{equation}\label{eq:gtwo}
	\sum_{i\in [1,a]}\sum_{j  \in \ztbtt}z_{\si,j}w_{j}=\sum_{j\in \ztbtt}w_{j}\sum_{i  \in [1,a]}z_{\si,j}=\sum_{j\in \ztbtt}w_{j}x_{j}~.
	\end{equation}
	In the first equality we interchanged the summations. In the second equality we used $\sum_{i  \in [1,a]}z_{\si,j}=\sum_{i' \in \ztbtt}z_{i',j}$ and further invoked condition 1 of the lemma. Now consider the second term in the final expression of \Cref{eq:gone},
	\begin{equation}\label{eq:gthree}
	\begin{split}
	\sum_{i\in [1,a]}\sum_{s_{i}\leq j  \leq s_{i+1}}z_{\si,j}(w_{s_{i}}-w_{s_{i+1}})&= \sum_{i\in [1,a]}(w_{s_{i}}-w_{s_{i+1}})\sum_{s_{i}\leq j  \leq s_{i+1}}z_{\si,j}
	= \sum_{i\in [1,a]}(w_{s_{i}}-w_{s_{i+1}})\\
	&= (w_{s_{1}}-w_{s_{x+1}})
	\leq \max_{j\in \ztbtt}w_{j}~.
	\end{split}
	\end{equation}
	The second equality follows by line 6 of the algorithm.	Condition 2 follows by combining equations \ref{eq:gone}, \ref{eq:gtwo} and \ref{eq:gthree}.
	
	{\bf Condition 3:} First we show that $z_{i,j}>0$ implies $i\leq j$. Consider $j \in \ztbtt$,
	\begin{enumerate}
		\item If $j\in \{s_{i}\}_{i\in [1,a]}$, in this case let $i \in [1,a]$ be such that $s_{i}=j$. Then by the second and third case in line 6 of the algorithm we have,
		$z_{i',j}>0$ implies $i'\in \{s_{i},s_{i-1}\}$. Further, using $s_{i-1}<s_{i}$ and $s_{i}=j$ we have $i' \leq j$.
		\item Else $j\in \ztbtt\backslash \{s_{i}\}_{i\in [1,a]}$ and in this case let $i \in [1,a]$ be such that $s_{i}<j<s_{i+1}$. Then by the first case in line 6 of the algorithm we have, $z_{i',j}>0$ implies $i'=s_{i}$. Further, using $s_{i}<j$ we have $i'<j$.
	\end{enumerate}
	Using the above implication we have,
	\begin{equation}
	\begin{split}
	\prod_{j\in \ztbtt}w_{j}^{\mmjj x_{j}}&=\prod_{j\in \ztbtt}w_{j}^{\mmjj \sum_{i\in \ztbtt}z_{i,j}}=\prod_{i\in \ztbtt}\prod_{j\in \ztbtt}w_{j}^{\mmjj z_{i,j}}\leq \prod_{i\in \ztbtt}\prod_{j\in \ztbtt}w_{i}^{\mmjj z_{i,j}}
	\end{split}
	\end{equation}
	In the first equality we used $x_{j}=\sum_{i\in \ztbtt}z_{i,j}$ for all $j \in \ztbtt$ (Condition 1). In the final inequality, we used the result $z_{i,j}>0$ implies $i\leq j$ and further combined it with the assumption at the begining of the proof, that is, $w_{i}\geq w_{j}$ for all $i,j \in \ztbtt$ and $i \leq j$.
\end{proof}



\renewcommand{\bttpo}{(\btt+1)}
\renewcommand{\bSp}{\textbf{B}}
\renewcommand{\bS}{\textbf{C}}
\renewcommand{\boo}{t}


\begin{proof}[Proof of \Cref{lem:create}] 
	Define $\phi_{0}\defeq \sum_{i \in [1,\boo]} \bSp_{i,0}$. In the following we provide the proof for each case.
	
	{\bf Condition 1:} For each $i\in [1,\boo]$, $\bSp'_{i,j} =\bS_{i,j}$ for all $j\in \ztbtt$ and the first condition holds.
	
	{\bf Condition 2:} Note $\bSp'$ is initialized to a zero matrix (Line 4). Further for any $i\in [\boo+1,\boo+\newk]$ let $j \in \ztbtt$ be such that $i=\boo+1+j$, then the algorithm only updates the $\bSp'_{\boo+1+j,j}$'th entry in the $i$'th row and keeps rest of the entries unchanged. Therefore the second condition holds.
	
	{\bf Condition 3:} For each $i\in [\boo+1,\boo+\newk]$ let $j \in \ztbtt$ be such that $i=\boo+1+j$, then $\sum_{j'\in \ztbtt}\bSp'_{i,j'}=\bSp'_{\boo+1+j,j}=\sum_{i' \in \otboo}(\bSp_{i',j}-\bS_{i',j})=\phi_{j}-\sum_{i' \in [1,\boo]}\bS_{i',j}$. The first equality holds because of the Condition 2. The third equality follows from the Line 8 of the algorithm. The last equality holds because $\bSp \in \bZfrac$ and we have $\sum_{i \in [1,\ell]}\bSp_{i,j}=\phi_{j}$.
	
	{\bf Condition 4:} Here we provide the proof for $\bSp' \in \textbf{Z}^{\phi,frac}_{\bR'}$. %Recall from \Cref{def:bzfrac}, 
	For any $j\in \ztbtt$, we first show that $\sum_{i\in [1,\boo+\newk]}\bSp'_{i,j}=\phi_{j}$.
	\begin{align*}
	\sum_{i\in [1,\boo+\newk]}\bSp'_{i,j}&=\sum_{i \in [1,\boo]}\bSp'_{i,j}+\sum_{i \in [\boo+1,\boo+\newk]}\bSp'_{i,j}
	=\sum_{i \in [1,\boo]}\bS_{i,j}+\bSp'_{\boo+1+j,j}\\
	&=\sum_{i \in [1,\boo]}\bS_{i,j}+\phi_{j}-\sum_{i \in [1,\boo]}\bS_{i,j}=\phi_{j}\\
	\end{align*}
	The second equality follows because $\bSp'_{i,j}=\bS_{i,j}$ for all $i\in [1,\boo]$ and $j\in \ztbtt$ (Line 6) and $\sum_{i \in [\boo+1,\boo+\newk]}\bSp'_{i,j}=\bSp'_{\boo+1+j,j}$ (Condition 2). The third equality follows from the Condition 3.
	
	We next show that $\sum_{i\in [1,\boo+\newk]}\pvec_{i} \left( \sum_{j\in \ztbtt}\bSp'_{i,j} \right) \leq 1$.
	\begin{equation}
	\begin{split}
	\sum_{i\in [1,\boo+\newk]}\pvec_{i} \left( \sum_{j\in \ztbtt}\bSp'_{i,j} \right)&=\sum_{i\in [1,\boo]}\pvec_{i} \left( \sum_{j\in \ztbtt}\bSp'_{i,j} \right)+ \sum_{j\in \ztbtt}\pvec_{\boo+1+j} \bSp'_{\boo+1+j,j}\\
	&=\sum_{i\in [1,\boo]}\pvec_{i} \left( \sum_{j\in \ztbtt}\bS_{i,j} \right)+ \sum_{j\in \ztbtt}\frac{\sum_{i \in \otboo}(\bSp_{ij}-\bS_{ij})\pvec_{i}}{\sum_{i \in \otboo}(\bSp_{ij}-\bS_{ij})} \left(\sum_{i \in \otboo}(\bSp_{i,j}-\bS_{i,j}) \right)\\
	&=\sum_{i\in [1,\boo]}\pvec_{i} \left( \sum_{j\in \ztbtt}\bS_{i,j} \right)+ \sum_{j\in \ztbtt}\sum_{i \in \otboo}(\bSp_{ij}-\bS_{ij})\pvec_{i}\\
	&=\sum_{i\in [1,\boo]}\pvec_{i} \left( \sum_{j\in \ztbtt}\bSp_{i,j} \right) \leq 1\\
	\end{split}
	\end{equation}
	In the first equality, we divided the summation into two parts and for the second part we used Condition 3. In the second equality we used Line 7 and 8 of the algorithm. In the third and fourth equality we simplified the expression. In the final inequality we used $\bSp \in \bZfrac$.
	
	Combining all the conditions together we have $\bSp' \in \textbf{Z}^{\phi,frac}_{\bR'}$. In the remainder we show that $\sum_{i \in [1,\boo+\newk]} \sum_{j \in \ztbtt} \bSp'_{i,j}=\sum_{i \in [1,\boo]} \sum_{j \in \ztbtt} \bSp_{i,j}$.
	
	Recall we already showed that $\sum_{i\in [1,\boo+\newk]}\bSp'_{i,j}=\phi_{j}$ for all $j \in \ztbtt$. Recall $\phi_{0}= \sum_{i \in [1,\boo]} \bSp_{i,0}$ and $\bSp \in \bZfrac$ implies $\phi_{j}=\sum_{i\in [1,\boo]}\bSp_{i,j}$ for all $j \in [1,\btt]$. Therefore we have, $$\sum_{i \in [1,\boo+\newk]} \sum_{j \in \ztbtt} \bSp'_{i,j}=\sum_{i \in [1,\boo]} \sum_{j \in \ztbtt} \bSp_{i,j}$$
	
	{\bf Condition 5:} We first provide the explicit expressions for $\bg(\bSp')$ and $\bg(\bSp)$ below: 
	$$ \bg(\bSp')=\left(\prod_{i \in \otboo}\pp_i^{(\bSp' \mvec)_i}\frac{\expo{(\bSp' \onevec)_i \log (\bSp' \onevec)_i}}{\prod_{j \in \ztbtt}\expo{\bSp'_{ij}\log \bSp'_{ij}}}\right)\left(\prod_{j \in \ztbtt} \pp_{\boo+1+j}^{\nn_j\bSp'_{\boo+1+j,j} }\cdot 1\right)$$
	$$ \bg(\bSp)=\prod_{i \in \otboo}\left(\pp_i^{(\bSp \mvec)_i}\frac{\expo{(\bSp \onevec)_i \log (\bSp \onevec)_i}}{\prod_{j \in \ztbtt}\expo{\bSp_{ij}\log \bSp_{ij}}}\right)$$
	Note in the expression for $\bg(\bSp')$ we used Condition 2. In the above two definitions for $\bg(\bSp')$ and $\bg(\bSp)$, we refer to the expression involving $\pvec_{i}$'s as the probability term and the rest as the counting term. We start the analysis of Condition 5 by first bounding the probability term:
	\begin{equation}\label{eq:probterm}
	\begin{split}
	\prod_{i \in \otboo}&\pp_i^{(\bSp \mvec)_{i}}=\left(\prod_{i \in \otboo}\pp_i^{(\bSp' \mvec)_i}\right)\left(\prod_{i \in \otboo}\pp_i^{\sum_{j \in \ztbtt}\nn_j(\bSp_{ij}-\bSp'_{ij})}\right)
	=\left(\prod_{i \in \otboo}\pp_i^{(\bSp' \mvec)_i}\right)\left(\prod_{j \in \ztbtt} \prod_{i \in \otboo}\pp_i^{\nn_j(\bSp_{ij}-\bSp'_{ij})}\right)\\
	&=\left(\prod_{i \in \otboo}\pp_i^{(\bSp' \mvec)_i}\right)\left(\prod_{j\in \ztbtt} \left(\prod_{i \in \otboo}\pp_i^{(\bSp_{ij}-\bSp'_{ij})}\right)^{\nn_j}\right)=\left(\prod_{i \in \otboo}\pp_i^{(\bSp' \mvec)_i}\right)\left(\prod_{j \in \ztbtt} \left(\prod_{i \in \otboo}\pp_i^{(\bSp_{ij}-\bS_{ij})}\right)^{\nn_j}\right)\\
	&\leq \left(\prod_{i \in \otboo}\pp_i^{(\bSp' \mvec)_i}\right)\left(\prod_{j \in \ztbtt} \left(\frac{\sum_{i \in \otboo}\pp_i(\bSp_{ij}-\bS_{ij})}{\sum_{i \in \otboo}(\bSp_{ij}-\bS_{ij})}\right)^{\nn_j\sum_{i \in \otboo}(\bSp_{ij}-\bS_{ij})}\right)\\
	&\leq \left(\prod_{i \in \otboo}\pp_i^{(\bSp' \mvec)_i}\right)\left(\prod_{j \in \ztbtt} \pp_{\boo+1+j}^{\nn_j\bSp'_{\boo+1+j,j}}\right)\\
	\end{split}
	\end{equation}
	The first three inequalities simplify the expression. The fourth equality follows because $\bSp'_{i,j} =\bS_{i,j}$ for all $i\in [1,\boo]$ and $j\in \ztbtt$. The fifth inequality follows from AM-GM inequality. The final expression above is the probability term associated with $\bSp'$ and the equation above shows that our rounding procedure only increases the probability term and it remains to bound the counting term.
	\begin{equation}\label{eq:countterm}
	\begin{split}
	\frac{\bg(\bSp')}{\bg(\bSp)} & \geq \prod_{i \in \otboo}\frac{\expo{(\bSp' \onevec)_i \log (\bSp' \onevec)_i-(\bSp \onevec)_{i} \log (\bSp \onevec)_{i}}}{\prod_{j \in \ztbtt}\expo{\bSp'_{ij}\log \bSp'_{ij}-\bSp_{ij}\log \bSp_{ij}}}\\
	&=\prod_{i \in \otboo}\frac{\expo{(\bS \onevec)_i \log (\bS \onevec)_i-(\bSp \onevec)_{i} \log (\bSp \onevec)_{i}}}{\prod_{j \in \ztbtt}\expo{\bS_{ij}\log \bS_{ij}-\bSp_{ij}\log \bSp_{ij}}}~.
	\end{split}
	\end{equation}
	Consider the numerator in the above expression, for each $i\in \otboo$ let $s_{i}\defeq(\bS \onevec)_i$, then
	\begin{equation}
	\begin{split}
	\prod_{i \in \otboo}\expo{(\bS \onevec)_i \log (\bS \onevec)_i-(\bSp \onevec)_{i} \log (\bSp \onevec)_{i}}&=\prod_{i \in \otboo}\expo{s_i \log s_i-(s_{i}+\alpha_{i}) \log (s_{i}+\alpha_{i})}\\
	&=\prod_{i \in \otboo}\expo{s_{i}\log \frac{s_{i}}{s_{i}+\alpha_{i}} -\alpha_{i}\log (s_{i}+\alpha_{i})}\\
	&\geq \prod_{i \in \otboo}\expo{s_{i}\frac{-\alpha_{i}}{s_{i}} -\alpha_{i}\log (s_{i}+\alpha_{i})}\\
	&\geq \expo{-O\left(\log (\sum_{i\in [1,\boo]}s_{i})\sum_{i\in \otboo}\alpha_{i} \right)}\\
	&\geq \expo{-O\left(\sum_{i\in \otboo}\alpha_{i} \log \logparam \right)}~.
	\end{split}
	\end{equation}
	In the third inequality we used $\log (1+x) \geq \frac{x}{1+x}$ for all $x \geq -1$. The final inequality follows because $\sum_{i\in [1,\boo]}s_{i} \leq\sum_{i\in [1,\boo]}(\bSp \onevec)_{i} \leq  \logparam$.
	Now consider the denominator in the above expression, let $\alpha_{i,j}=\bSp_{i,j}-\bS_{i,j}$ for all $i\in \otboo$ and $j\in \ztbtt$, then 
	\begin{equation}\label{eq:derive}
	\begin{split}
	\prod_{i \in \otboo}\prod_{j \in \ztbtt}\expo{\bS_{ij}\log \bS_{ij}-\bSp_{ij}\log \bSp_{ij}}&=\prod_{i \in \otboo}\prod_{j \in \ztbtt}\expo{\bS_{ij}\log \bS_{ij}-(\bS_{ij}+\alpha_{i,j})\log (\bS_{ij}+\alpha_{i,j})}\\
	&=\prod_{i \in \otboo}\prod_{j \in \ztbtt}\expo{\bS_{ij}\log \frac{\bS_{ij}}{\bS_{ij}+\alpha_{i,j}}-\alpha_{i,j}\log (\bS_{ij}+\alpha_{i,j})}\\
	&\leq \prod_{i \in \otboo}\prod_{j \in \ztbtt}\expo{-\alpha_{i,j}\log (\bS_{ij}+\alpha_{i,j})}\\ 
	&\leq \prod_{i \in \otboo}\prod_{j \in \ztbtt}\expo{-\alpha_{i,j}\log \alpha_{i,j}}\leq \expo{O\big(\log(\boo \times \btt)\sum_{i\in \otboo} \alpha_{i} \big)}\\
	& \leq \expo{O\left(\sum_{i\in \otboo} \alpha_{i} \log \logparam\right)}~.
	\end{split}
	\end{equation}
	In the third inequality we used $\alpha_{i,j} \geq 0$ and therefore $\bS_{ij}\log \frac{\bS_{ij}}{\bS_{ij}+\alpha_{i,j}} \leq 0$. In the fourth inequality we used $\log (\bS_{ij}+\alpha_{i,j}) \geq \log \alpha_{i,j}$. In the fifth inequality we used $\sum_{j \in \ztbtt} \alpha_{i,j}=\alpha_{i}$ for all $i\in \otboo$ and further $\sum_{i\in \otboo}\sum_{j \in \ztbtt}- \alpha_{i,j} \log  \alpha_{i,j}=\sum_{i\in \otboo}\alpha_{i} \left(\sum_{j \in \ztbtt} -\frac{\alpha_{i,j}}{\alpha_{i}} \log  \frac{\alpha_{i,j}}{\alpha_{i}}-\log \alpha_{i} \right) \leq \log (k+1)\sum_{i\in \otboo} \alpha_{i}  -\sum_{i\in \otboo}\alpha_{i} \log \alpha_{i}$. Now consider the term $-\sum_{i\in \otboo}\alpha_{i} \log \alpha_{i}$ and note that $-\sum_{i\in \otboo}\alpha_{i} \log \alpha_{i}=(\sum_{i\in \otboo}\alpha_{i})\left(-\sum_{i\in \otboo}\frac{\alpha_{i}}{\sum_{i\in \otboo}\alpha_{i}} \log \frac{\alpha_{i}}{\sum_{i\in \otboo}\alpha_{i}}-\log \sum_{i\in \otboo}\alpha_{i} \right)\leq (1+\log \boo)\sum_{i\in \otboo}\alpha_{i}$. The fifth inequality in \Cref{eq:derive} follows by combining the previous two derivations together. The final inequality follows because $\boo \times \btt \leq \logparam$.
	
	{\bf Condition 6:} This condition follows immediately from Line 7 of the algorithm.
\end{proof}




\renewcommand{\bSp}{\textbf{S}}
\renewcommand{\bS}{\textbf{A}}
\renewcommand{\boo}{\ell}

\begin{proof}[Proof of \Cref{lem:stepone}]
	In the following we provide the proof for the claims in the lemma.
	
	{\bf Condition 1:} Note $\bHone \subseteq \bH \cup [\ell+1,\ell+\newk]$, where $[\ell+1,\ell+\newk]$ are the indices corresponding to the new level sets created by the procedure $\algcreate$ (\Cref{alg:create}). Consider any $i \in \bHone$, then one the following two cases hold,
	\begin{enumerate}
		\item If $i \in \bH$, then by the first condition of \Cref{lem:create} we have $(\bSone \onevec)_{i}=(\ma \onevec)_{i}=\sum_{j\in \ztbtt} \ma_{i,j}=\sum_{j\in \ztbtt} \floor{\bSp_{i,j}} \in \Z$. 
		\item Else $i \in [\ell+1,\ell+\newk]$ and in this case we have $\sum_{i\in [1,\boo]}\ma_{i,j}=\sum_{i\in \bH}\ma_{i,j}+\sum_{i\in \bL}\ma_{i,j}=\sum_{i\in \bH}\floor{\bSp_{i,j}}+\floor{\sum_{i\in \bL}\bSp_{i,j}}\in \Z$. The second equality in the previous derivation follows from Line 7 and 8 of the algorithm. The previous derivation combined with third condition of \Cref{lem:create} we get,  $(\bSone \onevec)_{i}=\phi_{j}-\sum_{i\in [1,\boo]}\ma_{i,j}\in \Z$.
	\end{enumerate}
	$(\bSone \onevec)_{i} \in \Z$ in both the cases and the condition 1 follows.
	
	{\bf Condition 2:} This condition follows immediately from the fourth condition of \Cref{lem:create}.
	
	{\bf Condition 3:} Let $\alpha_{i}=\sum_{j\in \ztbtt}\bSp_{i,j} - \sum_{j\in \ztbtt}\ma_{i,j}$ for all $i\in [1,\boo]$. First we upper bound the term $\sum_{i\in \bH}\alpha_{i}$. Consider $\sum_{i\in \bH}\alpha_{i} \leq \sum_{i\in \bH} \sum_{j\in \ztbtt}\bSp_{i,j} \leq \tsqni$. The last inequality follows because of the constraint $\sum_{i\in [1,\boo]}\pvec_{i} \sum_{j\in \ztbtt}\bSp_{i,j} \leq 1$ ($\bSp \in \bZfrac$) and $\pvec_{i} >\tsqn$ for all $i \in \bH$. 
	
	We now upper bound the term $\sum_{i\in \bL}\alpha_{i}$. Consider $\sum_{i\in \bL}\alpha_{i}=\sum_{i\in \bL}\left(\sum_{j\in \ztbtt}\bSp_{i,j} - \sum_{j\in \ztbtt}\ma_{i,j}\right)=\sum_{j\in \ztbtt}\left(\sum_{i\in \bL}\bSp_{i,j} - \sum_{i\in \bL}\ma_{i,j}\right)$. Further $\sum_{i\in \bL}\ma_{i,j}=\floor{\sum_{i\in \bL}\bSp_{i,j}}$ for all $j\in \ztbtt$ (Line 8 of the algorithm) and we get $\sum_{i\in \bL}\alpha_{i} \leq k+1$. 
	
	Therefore $\sum_{i\in [\boo]}\alpha_{i}=\sum_{i\in \bH}\alpha_{i}+\sum_{i\in \bL}\alpha_{i} \leq \tsqni+k+1$ and combined with fifth condition \Cref{lem:create} we have, 
	$$\bg(\bSone) \geq \expo{-O\left(\left(\tsqni+k\right)\log \logparam \right)}\bg(\bSp) ~.$$
\end{proof}




\begin{proof}[Proof of \Cref{lem:steptwo}] 
	In the following we provide proof for all the conditions in the lemma.
	
	{\bf Condition 1:} For all $i \in [1,\boo+\newk]$, one of the following two conditions hold,
	\begin{enumerate}
		\item If $i \in \bHone$, then by the first condition of \Cref{lem:create} we have $(\bStwo \onevec)_{i}=(\bAone \onevec)_{i}=(\bSone \onevec)_{i} \in \Z$. The last expression follows from first condition of \Cref{lem:stepone}.
		\item Else $i \in \bLone$, then again by the first condition of \Cref{lem:create} we have $(\bStwo \onevec)_{i}=(\bAone \onevec)_{i}=\floor{(\bSone \onevec)_{i}} \in \Z$. The last equality follows from Line 15 of the algorithm.
	\end{enumerate}
	For all $i \in [1,\boo+\newk]$, we have $(\bStwo \onevec)_{i} \in \Z$ and therefore condition 1 holds.
	
	{\bf Condition 2:} This condition follows immediately from the second condition of \Cref{lem:create}.
	
	{\bf Condition 3:} This condition follows immediately from the fourth condition of \Cref{lem:create}.
	
	{\bf Condition 4:} Consider the term $\sum_{i \in [\boo+\newk+1,\boo+2\newk]} (\bStwo \onevec)_{i}$,
	\begin{equation}
	\begin{split}
	\sum_{i \in [\boo+\newk+1,\boo+2\newk]} (\bStwo \onevec)_{i}&=\sum_{i \in [1,\boo+2\newk]} (\bStwo \onevec)_{i} - \sum_{i \in [1,\boo+\newk]}(\bStwo \onevec)_{i}\\
	&=\sum_{j \in \ztbtt} \phi_{j} - \sum_{i \in [1,\boo+\newk]}(\bAone \onevec)_{i}\\
	&=\sum_{j \in \ztbtt} \phi_{j} - \left(\sum_{i \in \bHone}(\bAone \onevec)_{i}+\sum_{i \in \bLone}(\bAone \onevec)_{i} \right)\\
	&=\sum_{j \in \ztbtt} \phi_{j} - \left(\sum_{i \in \bHone}(\bSone \onevec)_{i}+\sum_{i \in \bLone} \floor{(\bSone \onevec)_{i}} \right) \in \Z
	\end{split}
	\end{equation}
	In the first equality we add and substract $\sum_{i \in [1,\boo+\newk]}(\bStwo \onevec)_{i}$ term. The first term in the second equality follows because $\sum_{i \in [1,\boo+2\newk]} (\bStwo \onevec)_{i}=\sum_{j \in \ztbtt} \sum_{i \in [1,\boo+2\newk]} \bStwo_{i,j}=\sum_{j \in \ztbtt} \phi_{j}$ and the last equality follows because $\bStwo \in \bZtwo$ (Condition 3). The second term in the second equality follows by the first condition of \Cref{lem:create}. In the third equality we divided the summation terms over $\bHone$ and $\bLone$. In the fourth equality we used Line 14 of the algorithm and further for any $i \in \bLone$ Line 15 implies $(\bAone \onevec)_{i}=\sum_{j\in \ztbtt}\bSone_{ij} \frac{\floor{(\bSone \onevec)_{i}}}{(\bSone \onevec)_{i}}=\floor{(\bSone \onevec)_{i}}$. Finally by first condition of \Cref{lem:stepone} we have $(\bSone \onevec)_{i} \in \Z$ for all $i \in \bHone$ and $\phi_{j} \in \Z$ for all $j \in \ztbtt$. Therefore, $\sum_{i \in [\boo+\newk+1,\boo+2\newk]} (\bStwo \onevec)_{i} \in \Z$ and the condition 4 holds.
	
	{\bf Condition 5:} For any $j \in \ztbtt$ we have,
	\begin{equation}
	\begin{split}
	\pvectwo_{\boo+\newk+1+j}&=\frac{\sum_{i \in [1,\boo+\newk]}(\bSone_{ij}-\bAone_{ij})\pvecone_{i}}{\sum_{i \in [1,\boo+\newk]}(\bSone_{ij}-\bAone_{ij})}
	=\frac{\sum_{i \in \bLone}(\bSone_{ij}-\bAone_{ij})\pvecone_{i}}{\sum_{i \in \bLone}(\bSone_{ij}-\bAone_{ij})}\\
	& \leq \tsqn \frac{\sum_{i \in \bLone}(\bSone_{ij}-\bAone_{ij})}{\sum_{i \in \bLone}(\bSone_{ij}-\bAone_{ij})} \leq \tsqn.
	\end{split}
	\end{equation}
	The first equality follows from the sixth condition of \Cref{lem:create}. The second equality follows because $\bSone_{i,j}=\bAone_{i,j}$ for all $i \in \bHone$ and $j \in \ztbtt$ (Line 14). The third inequality follows because $\bSone_{i,j} \geq \bAone_{i,j}$ for all $i \in \bLone$ and $j \in \ztbtt$ (Line 15) and further $\pvecone_{i} \leq \tsqn$ for all $i \in \bLone$ (Line 12).
	
	{\bf Condition 6:} For any $i \in [1,\boo+\newk]$, let $\alpha_{i}=\sum_{j \in \ztbtt}\bSone_{i,j} -\sum_{j \in \ztbtt}\bAone$. Note $\alpha_{i}=0$ for all $i\in \bHone$ (Line 14) and $\alpha_{i}= (\bSone \onevec)_{i}-\floor{(\bSone \onevec)_{i}} \leq 1$ for all $i \in \bLone$ (Line 15). Therefore $\sum_{i \in [1,\boo+\newk]} \alpha_{i}\leq |\bLone| \leq \boo+\newk$ and further combined with the fifth condition of \Cref{lem:create} we have $\bg(\bStwo) \geq \expo{-O\left((\boo+\btt)\log \logparam \right)} \bg(\bSone)$. Note by the third condition of \Cref{lem:stepone} we have $\bg(\bSone) \geq\expo{-O\left(\left(\tsqni+\btt \right)\log \logparam \right)} \bg(\bSp)$. Combining the previous two inequalities we get $\bg(\bStwo) \geq \expo{-O\left((\boo+\btt+\tsqni)\log \logparam \right)} \bg(\bSp)$ and condition 6 holds.
\end{proof}




\begin{proof}[Proof of \Cref{thm:stepthree}] In the following we provide proof for the two conditions of the theorem.
	
	{\bf Condition 1:} Here we provide the proof for the condition $\bSext \in \bZext$.
	\begin{enumerate}
		\item For all $i \in [1,\boo+2\newk]$, consider $(\bSext \onevec)_{i}$. If $i \in [1,\boo+\newk]$, then $(\bSext \onevec)_{i}=(\bStwo \onevec)_{i} \in \Z$. The first equality follows by line 22 of the algorithm and the last expression follows by first condition of \Cref{lem:steptwo}. Else $i \in [\boo+\newk+1,\boo+2\newk]$, let $j$ be such that $i=\boo+\newk+1+j$, then $(\bSext \onevec)_{i}= \sum_{j' \in \ztbtt}\bSext_{\boo+\newk+1+j,j'}=\sum_{j' \in \ztbtt}\left(\floor{\bStwo_{\boo+\newk+1+j,j'}}+z_{j,j'}\right)=\floor{\bStwo_{\boo+\newk+1+j,j}}+\sum_{j'\in \ztbtt}z_{j,j'} \in \Z$. The second equality follows by line 23 of the algorithm. The third equality follows from the second condition of \Cref{lem:steptwo}. Finally by the first condition of \Cref{lem:structured} we have $\sum_{j'\in \ztbtt}z_{j,j'} \in \{0,1\}$ for all $j \in \ztbtt$ and therefore $(\bSext \onevec)_{i} \in \Z$ for any $i \in [\boo+\newk+1,\boo+2\newk]$. 
		
		Combining the analysis of cases $i \in [1,\boo+\newk]$ and $i \in [\boo+\newk+1,\boo+2\newk]$ the condition 1 holds.
		
		\item For all $j \in \ztbtt$,
		\begin{equation}\label{eq:dddone}
		\begin{split}
		\sum_{i\in [1,\boo+2\newk]} \bSext_{i,j}&=\sum_{i\in [1,\boo+\newk]} \bSext_{i,j}+\sum_{i\in [\boo+\newk+1,\boo+2\newk]} \bSext_{i,j}\\
		&=\sum_{i\in [1,\boo+\newk]} \bStwo_{i,j}+\sum_{j' \in \ztbtt} \left(\floor{\bStwo_{\boo+\newk+1+j',j}}+z_{j',j}\right)~.
		\end{split}
		\end{equation}
		The second equality follows because $\bSext_{i,j}=\bStwo_{i,j}$ for all $i \in [1,\boo+\newk]$ (Line 22) and $\bSext_{i,j}=\floor{\bStwo_{\boo+\newk+1+j',j}}+z_{j',j}$ for all $i \in [\boo+\newk+1,\boo+2\newk]$ (Line 23).
		We next simplify the second term in the above expression.
		\begin{equation}\label{eq:dddtwo}
		\begin{split}
		\sum_{j' \in \ztbtt} \left(\floor{\bStwo_{\boo+\newk+1+j',j}}+z_{j',j}\right)&=\floor{\bStwo_{\boo+\newk+1+j,j}}+\sum_{j' \in \ztbtt}z_{j',j}
		=\floor{\bStwo_{\boo+\newk+1+j,j}}+x_{j}\\
		&=\bStwo_{\boo+\newk+1+j,j}=\sum_{i\in [\boo+\newk+1,\boo+2\newk]} \bStwo_{i,j}~.
		\end{split}
		\end{equation}
		In the first and final equality we used the second condition of \Cref{lem:steptwo} (Diagonal Structure). In the second equality we used the first condition of \Cref{lem:structured}. In the third equality we used the definition of $x_{j}$ (Line 19).
		Combining equations \ref{eq:dddone} and \ref{eq:dddtwo} we get,
		$$\sum_{i\in [1,\boo+2\newk]} \bSext_{i,j}=\sum_{i\in [1,\boo+2\newk]} \bStwo_{i,j} =\phi_{j}$$
		In the last inequality we used $\bStwo \in \bZtwo$.
		
		\item Let $\pvecext_{i}$ for all $i \in [1,\boo+2\newk]$ be the $i$'th element of $\bRext$. Consider $\sum_{i \in [1,\boo+2\newk]}\pvecext_{i}(\bSext \onevec)_{i}$, we have, 
		\begin{equation}\label{eq:derione}
		\begin{split}
		\sum_{i \in [1,\boo+2\newk]}&\pvecext_{i}(\bSext \onevec)_{i}=\sum_{i \in [1,\boo+2\newk]}\frac{\pvectwo_{i}}{1+\tsqn}(\bSext \onevec)_{i}\\
		%	&=\frac{1}{1+\sqrt{n}} \sum_{i \in [1,\boo+\newk+1]}\pvectwo_{i}(\bSext \onevec)_{i}+\frac{1}{1+\sqrt{n}}\sum_{i \in [\boo+\newk+1,\boo+2\newk]}\pvectwo_{i}(\bSext \onevec)_{i}\\
		&=\frac{1}{1+\tsqn} \sum_{i \in [1,\boo+\newk+1]}\pvectwo_{i}(\bStwo \onevec)_{i}+\frac{1}{1+\tsqn}\sum_{i \in [\boo+\newk+1,\boo+2\newk]}\pvectwo_{i}(\bSext \onevec)_{i}.
		\end{split}
		\end{equation}
		The first equality follows from Line 24 of the algorithm. In the second equality we divided the summation into two parts and used $\bSext_{i,j}=\bStwo_{i,j}$ for all $i \in [1,\boo+\newk+1]$ and $j \in \ztbtt$ (Line 22) for the first part. We now simplify the second part of the above expression.
		
		\begin{equation}\label{eq:deritwo}
		\begin{split}
		\sum_{i \in [\boo+\newk+1,\boo+2\newk]}\pvectwo_{i}(\bSext \onevec)_{i}%&=\sum_{j\in \ztbtt}\pvectwo_{\boo+\newk+1+j}\sum_{j'\in \ztbtt}\bSext_{\boo+\newk+1+j,j}\\
		&=\sum_{j\in \ztbtt}\pvectwo_{\boo+\newk+1+j}\sum_{j'\in \ztbtt}\left(\floor{\bStwo_{\boo+\newk+1+j,j'}}+z_{j,j'}\right)\\
		&=\sum_{j\in \ztbtt}w_{j}\left(\bStwo_{\boo+\newk+1+j,j}-x_{j}\right) +\sum_{j\in \ztbtt}w_{j}\sum_{j'\in \ztbtt}z_{j,j'}\\
		&\leq \sum_{j\in \ztbtt}w_{j}\left(\bStwo_{\boo+\newk+1+j,j}-x_{j}\right)+ \sum_{j\in \ztbtt} w_{j}x_{j}+\max_{j \in \ztbtt}w_{j}\\
		&=\sum_{i \in [\boo+\newk+1,\boo+2\newk]}\pvectwo_{i}(\bStwo \onevec)_{i}+\tsqn~.
		\end{split}
		\end{equation}
		In the first equality we expanded the $(\bSext \onevec)_{i}$ term. Further we used $\bSext_{\boo+\newk+1+j,j'}=\floor{\bStwo_{\boo+\newk+1+j,j'}}+z_{j,j'}$ for all $j,j' \in \ztbtt$ (Line 23). In the second equality we used the second condition of \Cref{lem:steptwo} (Diagonal Structure) and further combined it with definitions of $w_{j}$ and $x_{j}$ from Line 19 of the algorithm. The third inequality follows from second condition of \Cref{lem:structured}. In the final inequality we used $\max_{j \in \ztbtt}w_{j} \leq \tsqn$ that follows from the definition of $w_{j}$ and fifth condition of \Cref{lem:steptwo}. Further we combined it with $\bStwo_{\boo+\newk+1+j,j}=(\bStwo \onevec)_{i}$ that follows from the second condition of \Cref{lem:steptwo}.
		
		
		Combining equations \ref{eq:derione} and \ref{eq:deritwo} we have,
		$$\sum_{i \in [1,\boo+2\newk]}\pvecext_{i}(\bSext \onevec)_{i}\leq \frac{1}{1+\tsqn} \left(\sum_{i \in [1,\boo+2\newk]}\pvectwo_{i}(\bStwo \onevec)_{i}+\tsqn \right)\leq 1~.$$
		In the final inequality we used $\bStwo \in \bZtwo$ and therefore $\sum_{i \in [1,\boo+2\newk]}\pvectwo_{i}(\bStwo \onevec)_{i} \leq 1$.
	\end{enumerate}
	The condition 1 holds by combining the analysis of all the above three cases.
	
	{\bf Condition 2:} Recall the definition of $\bg(\bSext)$,
	\begin{align*}
	\bg(\bSext)=\prod_{i \in [1,\boo+2\newk]} \left({\pvecext_i}^{(\bSext \mvec)_i} \frac{\expo{(\bSext \onevec)_i \log (\bSext \onevec)_i}}{\prod_{j \in \ztbtt}\expo{\bSext_{ij}\log \bSext_{ij}}}\right)
	\end{align*}
	In the above expression consider the probability term,
	\begin{equation}\label{eq:done}
	\begin{split}
	\prod_{i \in [1,\boo+2\newk]} & {\pvecext_i}^{(\bSext \mvec)_i}=\prod_{i \in [1,\boo+2\newk]} \left(\frac{\pvectwo_i}{1+\tsqn} \right)^{(\bSext \mvec)_i}\\
	%&= \left(\left(1+\tsqn\right)^{-\sum_{i \in [1,\boo+2\newk]}(\bSext \mvec)_i} \right) \prod_{i \in [1,\boo+2\newk]} {\pvectwo_i}^{(\bSext \mvec)_i}\\
	&\geq  \expo{-O(\tsqn n)} \left(\prod_{i \in [1,\boo+\newk]} {\pvectwo_i}^{(\bSext \mvec)_i} \right)\left(\prod_{i \in [\boo+\newk+1,\boo+2\newk]} {\pvectwo_i}^{(\bSext \mvec)_i} \right)\\
	&=\expo{-O(\tsqn n)}\left(\prod_{i \in [1,\boo+\newk]} {\pvectwo_i}^{(\bStwo \mvec)_i} \right)\left(\prod_{i \in [\boo+\newk+1,\boo+2\newk]} {\pvectwo_i}^{(\bSext \mvec)_i} \right)\\
	%	&=\left(\prod_{i \in [1,\boo+\newk]} {\pvecext_i}^{(\bStwo \mvec)_i} \right)\left(\prod_{j\in \ztbtt} {\pvecext_{\boo+\newk+1+j}}^{\sum_{j'\in \ztbtt}\bSext_{j,j'} \mvec_{j'}} \right)\\
	%	&=\left(\prod_{i \in [1,\boo+\newk]} {\pvecext_i}^{(\bStwo \mvec)_i} \right)\left(\prod_{j\in \ztbtt} {\pvecext_{\boo+\newk+1+j}}^{\sum_{j'\in \ztbtt}(\floor{\bStwo_{\boo+\newk+1+j,j'}}+z_{j,j'}) \mvec_{j'}} \right)\\
	\end{split}
	\end{equation}
	In the first equality we used line 24 of the algorithm. In the second inequality we used $\sum_{i \in [1,\boo+2\newk]}(\bSext \mvec)_i=n$ that further implies $\left(1+\tsqn\right)^{-\sum_{i \in [1,\boo+2\newk]}(\bSext \mvec)_i} \geq \expo{-O(\tsqn n)}$. In the third equality we used $\bSext_{i,j}=\bStwo_{i,j}$ for all $i \in [1,\boo+\newk]$ and $j \in \ztbtt$ (Line 22).
	We now analyze the second product term in the final expression above,
	\begin{equation}\label{eq:dtwo}
	\begin{split}
	\prod_{i \in [\boo+\newk+1,\boo+2\newk]} & {\pvectwo_i}^{(\bSext \mvec)_i}=\prod_{j\in \ztbtt} {\pvectwo_{\boo+\newk+1+j}}^{\sum_{j'\in \ztbtt}\bSext_{\boo+\newk+1+j,j'} \mvec_{j'}}\\
	&=\prod_{j\in \ztbtt} {\pvectwo_{\boo+\newk+1+j}}^{\sum_{j'\in \ztbtt}\left(\floor{\bStwo_{\boo+\newk+1+j,j'}}+z_{j,j'} \right) \mvec_{j'}}\\
	&=\left( \prod_{j\in \ztbtt}{\pvectwo_{\boo+\newk+1+j}}^{\floor{\bStwo_{\boo+\newk+1+j,j}}} \right) \left(\prod_{j\in \ztbtt} {\pvectwo_{\boo+\newk+1+j}}^{\sum_{j'\in \ztbtt}z_{j,j'} \mvec_{j'}} \right).
	\end{split}
	\end{equation}
	The second equality follows from line 23 of the algorithm. The third equality follows from the second condition of \Cref{lem:steptwo} (Diagonal Structure).
	
	Now consider the second product term in the above expression.
	\begin{equation}\label{eq:dthree}
	\begin{split}
	\prod_{j\in \ztbtt} {\pvectwo_{\boo+\newk+1+j}}^{\sum_{j'\in \ztbtt}z_{j,j'} \mvec_{j'}}&=\prod_{j\in \ztbtt} w_{j}^{\sum_{j'\in \ztbtt}z_{j,j'} \mvec_{j'}} 
	\geq \prod_{j\in \ztbtt} w_{j}^{x_{j} \mvec_{j}}~.
	\end{split}
	\end{equation}
	In the first equality we used the definition of $w_{j}$ (Line 19). The second inequality follows from the third condition of \Cref{lem:structured}.
	
	Combining equations \ref{eq:dtwo}, \ref{eq:dthree} and further using $x_{j}=\bStwo_{\boo+\newk+1+j,j}-\floor{\bStwo_{\boo+\newk+1+j,j}}$ for all $j \in \ztbtt$ (Line 19) we have,
	\begin{equation}\label{eq:dfour}
	\prod_{i \in [\boo+\newk+1,\boo+2\newk]} {\pvectwo_i}^{(\bSext \mvec)_i}\geq \prod_{j\in \ztbtt} {\pvectwo_{\boo+\newk+1+j}}^{\bStwo_{\boo+\newk+1+j,j} \mvec_{j}}=\prod_{i \in [\boo+\newk+1,\boo+2\newk]} {\pvectwo_i}^{(\bStwo \mvec)_i}~.
	\end{equation}
	In the final inequality we used the second condition of \Cref{lem:steptwo} (Diagonal Structure).
	
	Combining equations \ref{eq:done} and \ref{eq:dfour} we have,
	$$\prod_{i \in [1,\boo+2\newk]} {\pvecext_i}^{(\bSext \mvec)_i} \geq \expo{-O(\tsqn n)} \prod_{i \in [1,\boo+2\newk]} {\pvectwo_i}^{(\bStwo \mvec)_i}$$
	
	Using the above expression we have,
	\begin{equation}\label{eq:eone}
	\begin{split}
	\frac{ \bg(\bSext)}{\bg(\bStwo)} &\geq \expo{-O(\tsqn n)} \prod_{i \in [1,\boo+2\newk]} \left( \frac{\expo{(\bSext \onevec)_i \log (\bSext \onevec)_i-(\bStwo \onevec)_i \log (\bStwo \onevec)_i}}{\prod_{j' \in \ztbtt}\expo{\bSext_{i,j'}\log \bSext_{i,j'}-\bStwo_{i,j'}\log \bStwo_{i,j'}}}\right)\\
	&=\expo{-O(\tsqn n)} \prod_{i \in [\boo+\newk+1,\boo+2\newk]} \left( \frac{\expo{(\bSext \onevec)_i \log (\bSext \onevec)_i-(\bStwo \onevec)_i \log (\bStwo \onevec)_i}}{\prod_{j' \in \ztbtt}\expo{\bSext_{i,j'}\log \bSext_{i,j'}-\bStwo_{i,j'}\log \bStwo_{i,j'}}}\right)\\
	&=\expo{-O(\tsqn n)} \prod_{i \in [\boo+\newk+1,\boo+2\newk]} \expo{(\bSext \onevec)_i \log (\bSext \onevec)_i-\sum_{j' \in \ztbtt}\bSext_{i,j'}\log \bSext_{i,j'}}~.
	\end{split}
	\end{equation}
	In the second equality we used $\bSext_{i,j}=\bStwo_{i,j}$ for all $i \in [1,\boo+\newk]$ and $j \in \ztbtt$ (Line 22). The third inequality follows by the second condition of \Cref{lem:steptwo} (Diagonal Structure). In the remainder of the proof we lower bound the term in the final expression.
	
	For each $i \in [\boo+\newk+1,\boo+2\newk]$ let $j \in \ztbtt$ be such that $i=\boo+\newk+1+j$, then $(\bSext \onevec)_i =\sum_{j' \in \ztbtt} (\floor{\bStwo_{\boo+\newk+1+j,j'}}+z_{j,j'}) = \floor{\bStwo_{\boo+\newk+1+j,j}} + \sum_{j' \in \ztbtt}z_{j,j'}$. The first equality follows from line 23 of the algorithm. The second equality follows by the second condition of \Cref{lem:steptwo} (Diagonal Structure). Using first condition of \Cref{lem:structured}, one of the following two cases hold,
	\begin{enumerate}
		\item If $\sum_{j' \in \ztbtt}z_{j,j'}=0$, then $z_{j,j'}=0$ for all $j' \in \ztbtt$. Using second condition of \Cref{lem:steptwo} (Diagonal Structure), we have $\bSext_{\boo+\newk+1+j,j'}=\floor{\bStwo_{\boo+\newk+1+j,j'}} + z_{j,j'}=0$ for all $j' \in \ztbtt$ and $j' \neq j$. Further note, $(\bSext \onevec)_i=\floor{\bStwo_{\boo+\newk+1+j,j}} + \sum_{j' \in \ztbtt}z_{j,j'}=\bSext_{\boo+\newk+1+j,j}$. Combining previous two equalities we have,
		$(\bSext \onevec)_i \log (\bSext \onevec)_i-\sum_{j' \in \ztbtt}\bSext_{i,j'}\log \bSext_{i,j'}=0$. Therefore,
		\begin{equation}\label{eq:etwo}
		\expo{(\bSext \onevec)_i \log (\bSext \onevec)_i-\sum_{j' \in \ztbtt}\bSext_{i,j'}\log \bSext_{i,j'}} \geq 1~.
		\end{equation}
		
		\item If $\sum_{j' \in \ztbtt}z_{j,j'}=1$, then $z_{j,j'} \in [0,1]_{\R}$ for all $j' \in \ztbtt$. Using second condition of \Cref{lem:steptwo} (Diagonal Structure), we have $\bSext_{i,j'}=\bSext_{\boo+\newk+1+j,j'}=\floor{\bStwo_{\boo+\newk+1+j,j'}} + z_{j,j'}=z_{j,j'}$ for all $j' \in \ztbtt$ and $j' \neq j$. Therefore, $\sum_{j' \in \ztbtt}\bSext_{i,j'}\log \bSext_{i,j'}=(\floor{\bStwo_{\boo+\newk+1+j,j}}+z_{j,j})\log (\floor{\bStwo_{\boo+\newk+1+j,j}}+z_{j,j})+\sum_{j' \neq j}z_{j,j'} \log z_{j,j'} \leq (\floor{\bStwo_{\boo+\newk+1+j,j}}+z_{j,j})\log (\floor{\bStwo_{\boo+\newk+1+j,j}}+z_{j,j})$. The final inequality follows because $z_{j,j'} \in [0,1]_{\R}$ and $z_{j,j'} \log z_{j,j'} \leq 0$ for all $j' \in \ztbtt$.
		
		Further note, $(\bSext \onevec)_i=\floor{\bStwo_{\boo+\newk+1+j,j}} + \sum_{j' \in \ztbtt}z_{j,j'}=\floor{\bStwo_{\boo+\newk+1+j,j}}+1$. Combining previous two inequalities we have,
		$(\bSext \onevec)_i \log (\bSext \onevec)_i-\sum_{j' \in \ztbtt}\bSext_{i,j'}\log \bSext_{i,j'} \geq (\floor{\bStwo_{\boo+\newk+1+j,j}}+1) \log (\floor{\bStwo_{\boo+\newk+1+j,j}}+1)-(\floor{\bStwo_{\boo+\newk+1+j,j}}+z_{j,j})\log(\floor{\bStwo_{\boo+\newk+1+j,j}}+z_{j,j}) \geq 0$. The last inequality follows because of the following: If $\floor{\bStwo_{\boo+\newk+1+j,j}}=0$, then the inequality follows because $z_{j,j} \in [0,1]_{\R}$ and $z_{j,j}\log z_{j,j} \leq 0$. Else $\floor{\bStwo_{\boo+\newk+1+j,j}} \geq 1$, in this case we use the fact that $x \log x$ is a monotonically increasing for $x \geq 1$. 
		
		Therefore 
		\begin{equation}\label{eq:ethree}
		\expo{(\bSext \onevec)_i \log (\bSext \onevec)_i-\sum_{j' \in \ztbtt}\bSext_{i,j'}\log \bSext_{i,j'}} \geq 1~.
		\end{equation}
	\end{enumerate}
	
	Combining equations \ref{eq:etwo} and \ref{eq:ethree}, for all $i \in [\boo+\newk+1,\boo+2\newk]$ we have,
	$$\expo{(\bSext \onevec)_i \log (\bSext \onevec)_i-\sum_{j' \in \ztbtt}\bSext_{i,j'}\log \bSext_{i,j'}} \geq 1~.$$
	Substituting previous inequality in \Cref{eq:eone} we get,
	$$\frac{ \bg(\bSext)}{\bg(\bStwo)} \geq \expo{-O(\tsqn n)}~.$$
	Further the condition 2 of the theorem follows by combining the above inequality with the sixth condition of \Cref{lem:steptwo}.
\end{proof}


==> rounding.tex <==
%!TEX root = neurips_2020.tex
\subsection{Rounding Algorithm}\label{subsec:algmain}
\renewcommand{\bttpo}{(\btt+1)}
\renewcommand{\bSp}{\textbf{B}}
\renewcommand{\bS}{\textbf{C}}
\renewcommand{\boo}{t}


The algorithm takes input $(\bSp,\bS,\bR,\phi)$ and creates new level sets $\bR'$ (lines 6-10). The solution $\bSp'$ outputted by the algorithm belongs to $\textbf{Z}^{\phi,frac}_{\bR'}$, has same column sums as $\bSp$ and the value $\bg(\bSp')$ is lower bounded by $\bg(\bSp)$. 

\begin{lemma}\label{lem:create}
Given a probability discretization set $\bR$ ($|\bR|=\boo$), profile $\phi$ (let $k$ be the number of distinct frequencies) and $\bSp \in \bZfrac \subseteq \R^{[1,\boo]\times \ztbtt}$ and $\bS\in \R^{[1,\boo]\times \ztbtt}$ such that $\bS_{i,j} \leq \bSp_{i,j}$ for all $i\in [1,\boo]$ and $j\in \ztbtt$. Let $\pvec_{i}$ be the $i$'th element of $\bR$.	There exists an algorithm that outputs a probability discretization set $\bR'$ and $\bSp'\in \R^{[1,\boo+\newk]\times \ztbtt}$ that satisfy the following conditions:
	\begin{enumerate}
		\item $\sum_{j\in \ztbtt}\bSp'_{i,j}=\sum_{j\in \ztbtt}\bS_{i,j}$ for all $i\in [1,\boo]$.
		\item For any $i \in [\boo+1,\boo+\newk]$ let $j \in \ztbtt$ be such that $i=\boo+1+j$ then $\bSp'_{\boo+1+j,j'}=0$ for all $j' \in \ztbtt$ and $j' \neq j$. (Diagonal Structure)
		\item For any $i\in [\boo+1,\boo+\newk]$ let $j \in \ztbtt$ be such that $i=\boo+1+j$, then $\sum_{j'\in \ztbtt}\bSp'_{i,j'}=\bSp'_{\boo+1+j,j}=\phi_{j}-\sum_{i' \in [1,\boo]}\bS_{i',j}$.
		\item $\bSp' \in \textbf{Z}^{\phi,frac}_{\bR'}$ and $\sum_{i \in [1,\boo+\newk]} \sum_{j \in \ztbtt} \bSp'_{i,j}=\sum_{i \in [1,\boo]} \sum_{j \in \ztbtt} \bSp_{i,j}$.
		%$\sum_{i\in [1,\boo+\btt]}\pvec_{i} \left( \sum_{j\in \ztbtt}\bSp'_{i,j} \right) \leq 1$.
		\item Let $\alpha_{i}\defeq \sum_{j\in \ztbtt}\bSp_{i,j} - \sum_{j\in \ztbtt}\bS_{i,j}$ for all $i\in [1,\boo]$ and $\logparam \defeq \max(\sum_{i \in [1,\boo]}(\bSp \onevec)_{i} , \boo \times \btt)$, then 
		$\bg(\bSp') \geq \expo{-O\left(  \sum_{i\in [1,\boo]} \alpha_{i}\log \logparam \right)} \bg(\bSp)~.$
		\item For any $j \in \ztbtt$, the new level sets have probability value equal to,
		$\pvec_{\boo+1+j}=\frac{\sum_{i \in \otboo}(\bSp_{ij}-\bS_{ij})\pvec_{i}}{\sum_{i \in \otboo}(\bSp_{ij}-\bS_{ij})}$.
	\end{enumerate}
	\end{lemma}

\newcommand{\rmin}{\textbf{r}_{min}}
\newcommand{\bZfracp}{\textbf{Z}^{\phi,frac}_{\bR'}}
\newcommand{\bZfracppp}{\textbf{Z}^{\phi,frac}_{\bR''}}
\newcommand{\mxext}{\mx^{ext}}
\newcommand{\bZfracext}{\textbf{Z}^{\phi,frac}_{\bRext}}
\newcommand{\bqext}{\bq^{ext}}
\begin{theorem}[Final rounding algorithm]
Given any $\mx \in \bZfrac$, there exists an algorithm that runs in polynomial time and returns a probability discretization set $\bRext$ and a solution $\mx'' \in \R$,
$$\bullet  \mx'' \in \textbf{Z}^{\phi}_{\bRext} \quad \quad  \bullet \bg(\mx'') \geq \exp(-O(k\log(\frac{1}{\rmin}+k^2))) \bg(\mx)~,$$
where $\rmin \defeq \min_{\ri \in \bR} \ri$ is the minimum non-zero probability value in $\bR$. Further the distribution $\bp'$ is the discrete pseudo distribution corresponding to $\mx'$ satisfies,
$$\Prob{\bp'', \phi} \geq \exp(-O(k\log \frac{1}{\rmin})) \bg(\mx)~.$$
	\end{theorem}
\begin{proof}
	The final rounding algorithm is a mixture of our matrix rounding algorithm and the create new level set algorithm. Consider $\mx \in \bZfrac$, by \Cref{lem:sparse} we can compute a solution $\mx' \in \bZfrac$ in polynomial time that satisfies: $\mx' \in \bZfrac$, $\bff(\mx') \leq \bff(\mx)$ and $\big|\{i \in [1,\ell]~|~[\mx'\1]_{i}  > 0\}\big| \leq k+1$. Let $S\defeq \{i \in [1,\ell]~|~[\mx'\1]_{i}  > 0\}$ and $\bR'\defeq \bR \backslash \{\ri \} _{i \in S}$. Let $\mx''$ be the submatrix that corresponds to the non-zero rows of matrix $\mx'$, then note that $\mx'' \in \bZfracp \subseteq \R^{[1,k+1]\times [0,k]}$ and satisfies $\bff(\mx'') \leq \bff(\mx)$. 
	
	By \Cref{lem}, we can compute a matrix $\ma'' \in \R^{[1,k+1]\times [0,k]}$ such that, for all $i \in [1,k+1]$ and $j \in [0,k]$ the following holds: $[\ma'' \vones]_{i} \in \Z$, $[\ma''^{\top}\vones ]_{j} \in \Z$, $\ma''_{ij} \leq \mx''_{ij}$ and $\sum_{i\in [1,k+1]} ([\mx''\vones]_{i}-[\ma''\vones]_{i}) \leq O(k)$.
	
	Now invoke the algorithm create new level set with input $(\mx'', \ma'',\bR')$, we get a probability discretization set $\bRext \subseteq \R^{[1,2k+2] \times [0,k]}$, a solution matrix $\mxext \in \bZfracext$ and the solution matrix $\mxext$ satisifes the conditions of the lemma.
	
	Since all the $\phi_{j}$ for all $j \in [0,k]$ are integer numbers, the conditions 1,2 and 3 of the lemma imply $[\mxext \vones]_{i} \in \Z$ for all $i \in [1,2k+2]$. Using condition 4 we have $\mxext \in \bZfracext$ and combined with the previous statement this implies $\mxext \in \za$. Further the function value $\bg(\mxext)$ satisfies,
	$\bg(\mxext) \geq \expo{-O\left(  \sum_{i\in [1,k+1]} \alpha_{i}\log \logparam \right)} \bg(\mx'')$, where $\logparam = \max(\sum_{i \in [1,k+1]} [\mx''\vones]_{i},(k+1)^2)$ and $\alpha_{i} = [\mx''\vones]_{i}-[\ma''\vones]_{i}$. First note that $\Delta \leq 1/\rmin + (k+1)^2$ because $\mx'' \in \bZfracp$ and therefore satisfies $\sum_{i \in [1,k+1]} \ri[\mx''\vones]_{i} \leq 1$ that further implies $\sum_{i \in [1,k+1]} [\mx''\vones]_{i} \leq 1/\rmin$. Now note that $\sum_{i\in [k+1]} \alpha_{i}=\sum_{i\in [k+1]} [\mx''\vones]_{i}-[\ma''\vones]_{i} \leq O(k)$ because of the above condition. Everything combined we get that, $\bg(\mxext) \geq \expo{-O\left(  k\log(1/\rmin + k^2) \right)} \bg(\mx'')$. Let $\bqext$ be the discrete pseudo distribution corresponding to $\mxext$ then we already know that \Cref{def} $\mxext \in \textbf{Z}^{\bqext,\phi}_{\bRext}$ and by the first condition of the \Cref{lem} we get that,
	$$\Prob{\bqext, \phi} \geq \exp(-O(k\log (\frac{1}{\rmin}+k^2))) \bg(\mx)~.$$
	
	
	
\end{proof}

==> writeup.tex <==
\input{anari}
We will prove the following theorem. 
	\begin{theorem}\label{thm:main}
		Suppose that $A\in \R_{\geq 0}^{n\times m}$. There exists $B\in \R_{\geq 0}^{n\times m}$, such that $A\geq B\geq 0$, $B\1\in \Z^n$, $B^\intercal \1\in \Z^m$, and $\sum_{i, j} (A_{ij}-B_{ij})\leq O(n+m)$.
	\end{theorem}
	We will first reduce it to the following form.
	\begin{lemma}\label{lem:mod}
		Suppose that $G=(V, E)$ is a bipartite graph and $k$ is a positive integer. There exists a subgraph $F\subseteq E$, such that $\deg_F(v)=0$ modulo $k$ for every vertex $v$, and $\card{E-F}\leq O(k\card{V})$.
	\end{lemma}
	\begin{proof}[Proof of \cref{lem:mod} $\implies$ \cref{thm:main}]
		If every entry of $A$ is an integer multiple of $1/k$ for some integer $k$, then it is enough to multiply $A$ by $k$ to get the adjacency matrix of some bipartite graph $G=(V, E)$. Then \cref{thm:main} directly follows from \cref{lem:mod}.
		
		Given an arbitrary $A$, we can round down each entry to the nearest integer multiple of $1/nm$. The total sum of entries in $A$ changes by at most $1$ (which can be absorbed in the $O(n+m)$ bound). Now we apply the argument in the above paragraph with $k=nm$.
	\end{proof}
	So it remains to prove \cref{lem:mod}. As our main tool, we will use a result from \cite{thomassen2014graph}. Roughly, this result says that as long as $G$ is sufficiently connected, we can choose a subgraph whose degrees are \emph{arbitrary} values modulo $k$. The exact statement is below:
	\begin{lemma}[\cite{thomassen2014graph}]\label{lem:connected}
		Suppose that $G=(V, E)$ is a bipartite $(3k-3)$-edge-connected graph. Suppose that $f:V \to \set{0, \dots, k-1}$ is an arbitrary function, with the restriction that the sum of $f$ on either side of the bipartite graph $G$ yields the same result modulo $k$. Then, there is a subgraph $F\subseteq E$, such that for each vertex $v$, $\deg_F(v)=f(v)$ modulo $k$.
	\end{lemma}
	Note that this result does not guarantee anything about $\card{E-F}$, even when $f$ is the zero function (it can actually return the empty subgraph in that case). We will fix that using a theorem of \cite{nash1961edge}. We will first prove \cref{lem:mod} with the extra assumption that $G$ is $6k$-edge-connected, and then prove the general case.
	\begin{proof}[Proof of \cref{lem:mod} when $G$ is $6k$-edge-connected]
		By a famous theorem due to \cite{nash1961edge}, a $6k$-edge-connected graph contains $3k$ edge-disjoint spanning trees. Let $H$ be the subgraph formed by these $3k$ edge-disjoint spanning trees. We will ensure that all edges outside $H$ are included in $F$; this way, we will automatically get that $\card{E-F}$ is bounded by the number of edges in $H$, which is at most $3k(\card{V}-1)=O(k\card{V})$.
		
		Let $H^c$ denote the complement of $H$ in $G$. Define the function $f:V\to\set{0, \dots, k-1}$ in the following way: let $f(v)$ be $-\deg_{H^c}(v)$ modulo $k$. Note that $f$ has the same sum on either side of the bipartite graph, modulo $k$. We will apply \cref{lem:connected} to the graph $H$ (which is $3k\geq (3k-3)$-edge-connected) and the function $f$. Then we take the union of the subgraph promised by \cref{lem:connected} and $H^c$ and output the result as $F$. Then $\deg_F(v)=\deg_{H^c}(v)+f(v)=0$ modulo $k$, for every vertex $v$. Note again that since we only deleted edges in $H$ to get $F$, the total number of edges we have removed can be at most $O(k\card{V})$.
	\end{proof}
	
	Now that we have proven \cref{lem:mod} for highly-connected graph, we prove it for the general case.
	
	\begin{proof}[Proof of \cref{lem:mod}]
		Since the input graph is arbitrary, we have no guarantee about connectivity.
		
		We will show that we can remove $O(k\card{V})$ edges from $G$ so that the remaining subgraph is a vertex-disjoint union of $6k$-edge-connected induced subgraphs. To do this, look at the connected components of $G$. Either they are all $6k$-edge-connected or at least one of them has a cut with $<6k$ edges. In the latter case, remove all edges of the small cut, and repeat. Every time we remove the edges of a cut, the number of connected components increases by $1$, so this can go on for at most $O(\card{V})$ iterations. In each iteration, at most $6k$ edges are removed, so the total number of removed edges is $O(k\card{V})$.		
		
		So by removing $O(k\card{V})$, we have transformed $G$ into a vertex-disjoint union of $6k$-edge-connected graphs. We simply apply the already-proved case of \cref{lem:mod} to each of these graphs to get our desired result for the arbitrary graph $G$.
	\end{proof}
\end{document}
